Model-based spectral coherence analysis

Recent data-driven efforts have utilized spectral decomposition techniques to uncover the geometric self-similarity of dominant motions in the logarithmic layer, and thereby validate the attached eddy model. In this paper, we evaluate the predictive capability of the stochastically forced linearized Navier-Stokes equations in capturing such structural features in turbulent channel flow at $Re_\tau=2003$. We use the linear coherence spectrum to quantify the wall-normal coherence within the velocity field generated by the linearized dynamics. In addition to the linearized Navier-Stokes equations around the turbulent mean velocity profile, we consider an enhanced variant in which molecular viscosity is augmented with turbulent eddy-viscosity. We use judiciously shaped white- and colored-in-time stochastic forcing to generate a statistical response with energetic attributes that are consistent with the result of direct numerical simulation (DNS). Specifically, white-in-time forcing is scaled to ensure that the two-dimensional energy spectrum is reproduced and colored-in-time forcing is shaped to match normal and shear stress profiles. We show that the addition of eddy-viscosity significantly strengthens the self-similar attributes of the resulting stochastic velocity field within the logarithmic layer and leads to an inner-scaled coherence spectrum. We use this coherence spectrum to extract the energetic signature of self-similar motions that actively contribute to momentum transfer and are responsible for producing Reynolds shear stress. Our findings support the use of colored-in-time forcing in conjunction with the dynamic damping afforded by turbulent eddy-viscosity in improving predictions of the scaling trends associated with such active motions in accordance with DNS-based spectral decomposition.

==> Tikz_common_styles.tex <==
%_______________________________________________________________
%
%     Tikz_common_styles
%
%     TikZ styles for drawing block diagrams.
%
%      Roy Smith,  15 July 2014
%
%_______________________________________________________________
\typeout{Reading Tikz styles:  Tikz_common_styles}
%
%   Block diagram styles
\tikzstyle{block} = [draw,rectangle,thick,minimum height=2em,minimum width=1.0cm,
                                top color=blue!10, bottom color=blue!10]%
\tikzstyle{sum} = [draw,circle,inner sep=0mm,minimum size=2mm]%
\tikzstyle{connector} = [->,thick]%
\tikzstyle{line} = [thick]%
\tikzstyle{branch} = [circle,inner sep=0pt,minimum size=1mm,fill=black,draw=black]%
\tikzstyle{guide} = []%
%
%   colours for various blocks
\tikzstyle{deltablock} = [block, top color=red!10, bottom color=red!10]%
\tikzstyle{controlblock} = [block, top color=green!10, bottom color=green!10]%
\tikzstyle{weightblock} = [block, top color=orange!10, bottom color=orange!10]%
\tikzstyle{clpblock} = [block, top color=cyan!10, bottom color=cyan!10]%
%
%  styles for dimming block components.
\tikzstyle{block_dim} = [draw,rectangle,thick,minimum height=2em,minimum width=2em,
                                color=black!15]%
\tikzstyle{sum_dim} = [draw,circle,inner sep=0mm,minimum size=2mm,color=black!15]%
\tikzstyle{connector_dim} = [->,thick,color=black!15]%
%
%    Graph styles
\tikzstyle{smalllabel} = [font=\footnotesize]%
\tikzstyle{axiswidth}=[semithick]%
\tikzstyle{axiscolor}=[color=black!50]%
\tikzstyle{help lines} =[color=blue!40,very thin]%
\tikzstyle{axes} = [axiswidth,axiscolor,<->,smalllabel]%
\tikzstyle{axis} = [axiswidth,axiscolor,->,smalllabel]%
\tikzstyle{tickmark} = [thin,smalllabel]%
\tikzstyle{plain_axes} = [axiswidth,smalllabel]%
\tikzstyle{w_axes} = [axiswidth,->,smalllabel]%
\tikzstyle{m_axes} = [axiswidth,smalllabel]%
\tikzstyle{dataplot} = [thick]%
%
%_______________________________________________________________


==> frameworkloop.tex <==
%_______________________________________________________________________________
%
%   tikz figure for inclusion in exercises:
%
%   clp_2dof_output_pert_config:  closed loop system with perturbed models.  This uses
%                                              and input perturbation and the 2-DOF structure used for
%                                              the satellite example.
%
%   Marcello Colombino, 4 May 2015
%
%_______________________________________________________________________________
%
% TikZ styles for drawing
%
\input{../figures/Tikz_common_styles}
%
%   set a filename for externalization
% \tikzsetnextfilename{clp_2dof_input_pert_config}
%
\noindent
\begin{tikzpicture}[scale=1, auto, >=stealth']

    \footnotesize

   % specify with respect to the plant
     \node[block, minimum height = 1cm, top color=red!20, bottom color=red!20] (sys0) {\begin{tabular}{c}linearized\\ flow dynamics\end{tabular}};     
     
     \node[block, minimum height = 1cm, top color=RoyalBlue!20, bottom color=RoyalBlue!20] (sys1) at ($(sys0.east) + (3.2cm, 1.5cm)$) {\begin{tabular}{c}mean-flow\\ equations\end{tabular}};
     
     \node[block, minimum height = 1cm, top color=RoyalBlue!20, bottom color=RoyalBlue!20] (sys2) at ($(sys1.east) + (3.2cm, 1.3cm)$) {$\nu_T=cRe_\tau^2(k^2/\epsilon)$};

     
     \node[] (input-node) at ($(sys0.west) + (-2.0cm, 0cm)$) {};

     %\node[] (output-node) at ($(sys1.west) + (-4cm, 0cm)$) {$\mathrm{turbulent \atop drag}$};
     
     \node[] (in-node1) at ($(sys0.north) + (0.25cm, -0.14cm)$) {};
     
     \node[] (end-node0) at ($(sys0.south) + (-0.28cm, 0.12cm)$) {};
     
     \node[] (end-node1) at ($(sys0.south) + (-1.0cm, -0.8cm)$) {};

     %\node[] (mid1) at ($(sys2.east) + (2.3cm,0cm)$) {};
     
     \node[] (mid2) at ($(sys1.west) + (-2.45cm,0cm)$) {};
     
     \node[] (mid20) at ($(sys2.west) + (-1.95cm,0cm)$) {};
     
     \node[] (mid21) at ($(sys1.north) + (0.25cm, -0.14cm)$) {};
     
     \node[] (mid22) at ($(sys1.south) + (-0.28cm, 0.12cm)$) {};
     
     \node[] (mid23) at ($(sys1.south) + (-1.0cm, -0.8cm)$) {};
    % now link the nodes
    
    \draw [connector, thick] (input-node) -- node [midway, above] {\begin{tabular}{c}stochastic\\ forcing\end{tabular}} (sys0.west);
    
    \draw [connector, thick] (sys0.east) -| node [pos=0.42, above] {\begin{tabular}{c}second-order\\ statistics\end{tabular}} (sys2.south);
	
    %\draw [line, double] (sys2.east) -- node [midway, above] {$\mathrm{turbulent \atop mean\ viscosity}$} (mid1.east);

    %\draw [connector, double] (mid1.east) |- (sys1.east);
    
    \draw [line, thick] (sys2.west) -- node [midway, above] {\begin{tabular}{c}turbulent\\ viscosity\end{tabular}} (mid20.east);

    \draw [line, thick] (mid20.east) -- (mid21);

    \draw [connector, thick] (mid22) -- (mid23);

    \draw [line, thick] (sys1.west) -- node [midway, above] {\begin{tabular}{c}turbulent\\ mean velocity\end{tabular}} (mid2.east);

    \draw [line, thick] (mid2.east) -- (in-node1);

    \draw [connector, thick] (end-node0) -- (end-node1);

\end{tikzpicture}
%_______________________________________________________________________________

